A stellar evolutionary grid for binary population synthesis: from the main sequence to helium ignition

Mass changes due to strong stellar winds and binary mass transfer have a dramatic impact on the consequent evolution of stars. This is generally not accounted for in population synthesis codes which are built using single star evolution models from full stellar evolution codes. We produce a new grid of models using the 1D stellar evolution code \textit{MESA} which includes models with a range of core mass fractions, at each total stellar mass, evolved from core hydrogen exhaustion to the onset of core helium burning. The model grid is used to produce an interpolation table, designed for use in population synthesis codes such as \textit{binary\_c}. We test the interpolation table with a simple integration algorithm to evaluate its capability of reproducing accurate evolutionary tracks. We test our method for stellar masses in the range $M=1-16~\mathrm{M}_\odot$ and show that it successfully reproduces the Hertzpsrung-gap and giant branch lifetime, the core mass at helium ignition and the HR diagram.

==> abstract.tex <==
Mass changes due to strong stellar winds and binary mass transfer have a dramatic impact on the consequent evolution of stars.
This is generally not accounted for in population synthesis codes which are built using single star evolution models from full stellar evolution codes.
We produce a new grid of models using the 1D stellar evolution code \textit{MESA} which includes models with a range of core mass fractions, at each total stellar mass, evolved from core hydrogen exhaustion to the onset of core helium burning.
The model grid is used to produce an interpolation table, designed for use in population synthesis codes such as \textit{binary\_c}.
We test the interpolation table with a simple integration algorithm to evaluate its capability of reproducing accurate evolutionary tracks.
We test our method for stellar masses in the range $M=1-16~\Msun$ and show that it successfully reproduces the Hertzpsrung-gap and giant branch lifetime, the core mass at helium ignition and the HR diagram.

